Hardness Amplification for Dynamic Binary Search Trees

We prove direct-sum theorems for Wilber's two lower bounds [Wilber, FOCS'86] on the cost of access sequences in the binary search tree (BST) model. These bounds are central to the question of dynamic optimality [Sleator and Tarjan, JACM'85]: the Alternation bound is the only bound to have yielded online BST algorithms beating $\log n$ competitive ratio, while the Funnel bound has repeatedly been conjectured to exactly characterize the cost of executing an access sequence using the optimal tree [Wilber, FOCS'86, Kozma'16], and has been explicitly linked to splay trees [Levy and Tarjan, SODA'19]. Previously, the direct-sum theorem for the Alternation bound was known only when approximation was allowed [Chalermsook, Chuzhoy and Saranurak, APPROX'20, ToC'24]. We use these direct-sum theorems to amplify the sequences from [Lecomte and Weinstein, ESA'20] that separate between Wilber's Alternation and Funnel bounds, increasing the Alternation and Funnel bounds while optimally maintaining the separation. As a corollary, we show that Tango trees [Demaine et al., FOCS'04] are optimal among any BST algorithms that charge their costs to the Alternation bound. This is true for any value of the Alternation bound, even values for which Tango trees achieve a competitive ratio of $o(\log \log n)$ instead of the default $O(\log \log n)$. Previously, the optimality of Tango trees was shown only for a limited range of Alternation bound [Lecomte and Weinstein, ESA'20].

==> figs/charging-cases.tex <==
\begin{figure}[h]
\centering

\newcommand{\access}[2]{\node[cross] (p#2) at (#1,#2) {};}
\newcommand{\nodeAbove}[2]{\node[above=0mm of #1] {#2};}
\newcommand{\added}[3]{
    \node[dot] (q#1#2) at (#1,#2) {};
    \nodeAbove{q#1#2}{#3}
}
\begin{tikzpicture}[scale=0.6]
\draw[lightgray] (2,0) rectangle (6,5);
\access{4}{0}
\access{0}{1}
\access{2}{2}
\access{6}{3}
\access{1}{4}
\access{3}{5}
\access{5}{6}
\added{0}{2}{a}
\added{2}{3}{c}
\added{4}{3}{a}
\added{0}{4}{a,b}
\added{1}{5}{b}
\added{2}{5}{a,b}
\added{3}{6}{b}
\added{4}{6}{a,b}
\end{tikzpicture}

\caption{Added points of $\protect\addUp(P)$ labeled with their type(s) from Lemma~\ref{lemma:highest-or-rightmost}. The \zr{} corresponding to the type-c point is drawn in gray.}\label{fig:charging-cases}
\end{figure}


==> figs/domination-idea.tex <==
\begin{figure}[h]
\centering
\newcommand{\diskColor}{gray}
\newcommand{\shadowColor}{lightgray}
\newcommand{\bottom}{-2}
\newcommand{\funnel}[3]{
    \fill[gray] (#1,#2) circle (3mm);
    \node at (#1,#2) (C) {};
    \node[above=0mm of C] {#3};
}
\newcommand{\funnelL}[3]{
    \fill[lightgray] (#1,#2) rectangle (#3,\bottom);
    \funnel{#1}{#2}{$\ttL$}
}
\newcommand{\funnelR}[3]{
    \fill[lightgray] (#1,#2) rectangle (#3,\bottom);
    \funnel{#1}{#2}{$\ttR$}
}
\newcommand{\access}[2]{\node[cross] (p#2) at (#1,#2) {};}
\newcommand{\pointSet}{
\access{3}{-1}
\access{8}{0}
\access{5}{1}
\access{2}{2}
\access{6}{3}
\access{9}{4}
\access{7}{5}
\access{4}{6}
\access{1}{7}
\node[above=0mm of p6] {$p$};
\node[right=1mm of p2] {$q$};
\draw[dashed, thin] (5.5,\bottom) -- (5.5,8);
}

\setlength{\tabcolsep}{5mm}
\begin{tabu}{c|c|c}
%\toprule
\begin{tikzpicture}[scale=0.5]
\pointSet{}
\draw [decorate,decoration={brace,amplitude=2mm},yshift=5mm]
(0.8,7) -- (5.2,7) node [midway,yshift=4mm] {from $\xL$};
\draw [decorate,decoration={brace,amplitude=2mm},yshift=5mm]
(5.8,7) -- (9.2,7) node [midway,yshift=4mm] {from $\xR$};
%\draw[dashed, gray] (p6) -- (4,\bottom);
\end{tikzpicture}&
\begin{tikzpicture}[scale=0.5]
\funnelL{3}{-1}{0.5}
\funnelL{2}{2}{0.5}
\funnelR{5}{1}{5.5}
\pointSet{}
%\draw[dashed, gray] (p6) -- (4,\bottom);
\end{tikzpicture}&
\begin{tikzpicture}[scale=0.5]
\funnelL{3}{-1}{0.5}
\funnelL{2}{2}{0.5}
\funnelR{5}{1}{9.5}
\funnelR{6}{3}{9.5}
\funnelR{7}{5}{9.5}
\pointSet{}
%\draw[dashed, gray] (p6) -- (4,\bottom);
\draw[dashed] (6.5,4.3) circle (2cm);
\node[text width=2cm,align=left] at (8.5,7.7) {\footnotesize completely new group of funnel points};
\end{tikzpicture}\\
geometric view of $\x$&
funnel of $p$ in $G_{\xL}$&
funnel of $p$ in $G_{\x}$\\
&(before interleaving)&(after interleaving)\\
\end{tabu}

\caption{Interleaving sequences $\xL=(3,5,2,4,1)$ and $\xR=(8,6,9,7)$ into $X=(3,8,5,2,6,9,7,4,1)$. The contribution of $p$ to $\Funnel(\xL)$ is 3, while the contribution of $p$ to $\Funnel(\x)$ is 4.}\label{fig:domination-idea}
\end{figure}


==> figs/hor-flip.tex <==
\begin{figure}[h]
\centering
\newcommand{\diskColor}{gray}
\newcommand{\shadowColor}{lightgray}
\newcommand{\bottom}{0}
\newcommand{\funnel}[3]{
    \fill[gray] (#1,#2) circle (3mm);
    \node at (#1,#2) (C) {};
    \node[above=0mm of C] {#3};
}
\newcommand{\funnelL}[2]{
    \fill[lightgray] (#1,#2) rectangle (-0.5,\bottom);
    \funnel{#1}{#2}{$\ttL$}
}
\newcommand{\funnelR}[2]{
    \fill[lightgray] (#1,#2) rectangle (8.5,\bottom);
    \funnel{#1}{#2}{$\ttR$}
}

\newcommand{\access}[2]{\node[cross] (p#2) at (#1,#2) {};}
$
\vcenter{\hbox{
\begin{tikzpicture}[scale=0.5]
\funnelL{3}{3}
\funnelL{2}{7}
\funnelL{1}{8}
\funnelR{5}{4}
\funnelR{7}{6}
\fill[\shadowColor] (-0.5,\bottom) rectangle (8.5,1);
\access{4}{1}
\access{6}{2}
\access{3}{3}
\access{5}{4}
\access{1}{5}
\access{7}{6}
\access{2}{7}
\access{1}{8}
\access{4}{9}
\access{6}{10}
\access{3}{11}
\node[above=0mm of p9] {$p$};
%\draw[dashed, gray] (p1) -- (p9);
\end{tikzpicture}
}}
\quad
\longleftrightarrow
\quad
\vcenter{\hbox{
\begin{tikzpicture}[scale=0.5]
\funnelR{5}{3}
\funnelR{6}{7}
\funnelR{7}{8}
\funnelL{3}{4}
\funnelL{1}{6}
\fill[\shadowColor] (-0.5,\bottom) rectangle (8.5,1);
\access{4}{1}
\access{2}{2}
\access{5}{3}
\access{3}{4}
\access{7}{5}
\access{1}{6}
\access{6}{7}
\access{7}{8}
\access{4}{9}
\access{2}{10}
\access{5}{11}
\node[above=0mm of p9] {$p$};
%\draw[dashed, gray] (p1) -- (p9);
\end{tikzpicture}
}}
$

\caption{Flipping the geometric view horizontally conserves the contribution $f(P,p)$ of each point: the only change is that the labels of the funnel points flip between $\ttL$ and $\ttR$.}\label{fig:hor-flip}
\end{figure}


==> figs/irb.tex <==
\begin{figure}[h]
\centering

\newcommand{\access}[2]{\node[cross] (p#2) at (#1,#2) {};}
\newcommand{\added}[2]{\node[dot] (q#2) at (#1,#2) {};}
\setlength{\tabcolsep}{8mm}
\begin{tabu}{cc}
\begin{tikzpicture}[scale=0.5]
\access{4}{0}
\access{0}{1}
\access{2}{2}
\access{6}{3}
\access{1}{4}
\access{3}{5}
\access{5}{6}
\added{0}{2}
\added{2}{3}
\added{4}{3}
\added{0}{4}
\added{1}{5}
\added{2}{5}
\added{3}{6}
\added{4}{6}
\end{tikzpicture}&
\begin{tikzpicture}[scale=0.5]
\access{4}{0}
\access{0}{1}
\access{2}{2}
\access{6}{3}
\access{1}{4}
\access{3}{5}
\access{5}{6}
\added{4}{1}
\added{4}{2}
\added{2}{4}
\added{6}{4}
\added{4}{5}
\added{6}{5}
\added{6}{6}
%\added{}{}
%\added{}{}
%\added{}{}
\end{tikzpicture}\\[2mm]
$\upIRB(P) = |\addUp(P)| = 8$&
$\downIRB(P) = |\addDown(P)| = 7$\\
\end{tabu}

\caption{Running Algorithm~\ref{alg:up-greedy} (and the analogous algorithm on the right) to compute $\protect\upIRB(P)$ and $\protect\downIRB(P)$}\label{fig:irb}
\end{figure}


==> figs/rects.tex <==
\begin{figure}[h]
\centering

\newcommand{\access}[2]{\node[cross] (p#2) at (#1,#2) {};}
\setlength{\tabcolsep}{5mm}
\begin{tabu}{cc}
\begin{tikzpicture}[scale=0.5]
\draw[gray] (1,1) rectangle (3,4);
\access{1}{1}
\node[left=0mm of p1] {$p$};
\access{3}{4}
\node[right=0mm of p4] {$q$};
\access{0}{3}
\end{tikzpicture}&
\begin{tikzpicture}[scale=0.5]
\draw[gray] (1,1) rectangle (4,3);
\access{1}{3}
\node[left=0mm of p3] {$r$};
\access{4}{1}
\node[right=0mm of p1] {$s$};
\access{2}{2}
\end{tikzpicture}\\
$\rect{pq}$ is empty&
$\rect{rs}$ is \emph{not} empty\\
\end{tabu}

\caption{some axis-aligned rectangles}\label{fig:rects}
\end{figure}


==> figs/separation-seq.tex <==
\begin{figure}[h]
\centering
\newcommand{\access}[2]{\node[cross] (p#2) at (#1,#2) {};}
\newcommand{\Szero}[3]{
\access{1+#1}{1+#2}
\access{4+#1}{2+#2}
\access{2+#1}{3+#2}
\access{8+#1}{4+#2}
\draw [decorate,decoration={brace,amplitude=2mm},xshift=-4mm,yshift=0pt]
(1,0.8+#2) -- (1,4.2+#2) node [midway,left,xshift=-2mm] {#3};
}
\newcommand{\customDots}[3]{
\node at (-0.5,1.8+#2) {$\vdots$};
\node at (4.5+#1,1.85+#2) {#3};
}
\newcommand{\group}[3]{
\Szero{#1}{#2}{#3}
\customDots{#1}{#2+4}{$\vdots$}
\Szero{#1}{#2+6}{#3}
}

\begin{tikzpicture}[scale=0.3]
\draw[step=1cm,lightgray,thin] (1,1) grid (16,34);
%\Szero{0}{0}{$S_0$}
\group{0}{0}{$S_0$}
\group{1}{10}{$S_1$}
\customDots{4.5}{21}{\reflectbox{$\ddots$}}
\group{8}{24}{$S_{n/2}$}
\end{tikzpicture}

\caption{A schematic view of sequence $\xTilde$ for $k=2$. Each part $S_i$ is made of $K=2^k=4$ accesses. There are $n=2^K=16$ distinct keys and the length of $\xTilde$ is $m=(16/2+1)nK=576$.}\label{fig:separation-seq}
\end{figure}


==> figs/time-reversal.tex <==
\begin{figure}[h]
\centering
\newcommand{\access}[2]{
\node[cross] (p#2) at (#1,#2) {};
%\node[gray, right=0mm of p1] {$({\color{black}{{#1}}},#2)$};
}
\setlength{\tabcolsep}{10mm}
\begin{tabu}{cc}
\begin{tikzpicture}[scale=0.4]
\access{0}{0}
\access{4}{1}
\node[right=0mm of p1] {$p$};
\access{1}{2}
\access{3}{3}
\access{6}{4}
\access{5}{5}
\access{2}{6}
\end{tikzpicture}&
\begin{tikzpicture}[scale=0.4]
\access{0}{7}
\access{4}{6}
\node[right=0mm of p6] {$\rev{p}$};
\access{1}{5}
\access{3}{4}
\access{6}{3}
\access{5}{2}
\access{2}{1}
\end{tikzpicture}\\[1mm]
$P$ & $\rev{P}$\\
\end{tabu}
\caption{A point set and its time reversal}\label{fig:time-reversal}
\end{figure}


==> figs/ver-flip.tex <==
\begin{figure}[h]
\centering
\newcommand{\access}[3]{
    \node[cross] (p#2) at (#1,#2) {};
    \node[above=0mm of p#2] {#3};
}

\setlength{\tabcolsep}{10mm}
\begin{tabu}{cc}
%\toprule
\begin{tikzpicture}[scale=0.5]
\access{1}{1}{$0$}
\access{3}{2}{$1$}
\access{2}{3}{$2$}
\end{tikzpicture}&
\begin{tikzpicture}[scale=0.5]
\access{2}{1}{$0$}
\access{3}{2}{$1$}
\access{1}{3}{$1$}
\end{tikzpicture}\\
$\Funnel(P) = 0+1+2 = 3$&
$\Funnel(\rev{P}) = 0+1+1 = 2$\\
\end{tabu}

\caption{A minimal example such that $\Funnel(P) \neq \Funnel(\protect\rev{P})$ is $P=\{(1,1),(3,2),(2,3)\}$. Each access $p$ is labeled with its contribution $f(P,p)$ (left) or $f(\protect\rev{P},p)$ (right).}\label{fig:ver-flip}
\end{figure}


==> figs/zrect-formal.tex <==
\begin{figure}[h]
\centering

\newcommand{\access}[2]{\node[cross] (p#2) at (#1,#2) {};}
\begin{tikzpicture}[scale=0.5]
\draw[gray] (2,2) rectangle (7,6);
\access{4}{1}
\access{5}{2}
\access{2}{3}
\access{7}{4}
\access{1}{5}
\access{3}{6}
\access{8}{7}
\access{6}{8}
\node[above=0mm of p6] {$p$};
\node[left=0mm of p3] {$q$};
\node[below=0mm of p2] {$r$};
\node[right=0mm of p4] {$s$};
\end{tikzpicture}
\caption{A \zr{}. The relative order of points $p,q,r,s$ horizontally and vertically matters.}\label{fig:zrect-formal}
\end{figure}

